Consistency by Agreement in Zero-shot Neural Machine Translation

Generalization and reliability of multilingual translation often highly depend on the amount of available parallel data for each language pair of interest. In this paper, we focus on zero-shot generalization---a challenging setup that tests models on translation directions they have not been optimized for at training time. To solve the problem, we (i) reformulate multilingual translation as probabilistic inference, (ii) define the notion of zero-shot consistency and show why standard training often results in models unsuitable for zero-shot tasks, and (iii) introduce a consistent agreement-based training method that encourages the model to produce equivalent translations of parallel sentences in auxiliary languages. We test our multilingual NMT models on multiple public zero-shot translation benchmarks (IWSLT17, UN corpus, Europarl) and show that agreement-based learning often results in 2-3 BLEU zero-shot improvement over strong baselines without any loss in performance on supervised translation directions.

==> introduction.tex <==
\section{Introduction}

Machine translation (MT) has made remarkable advances with the advent of deep learning approaches \citep{bojar2016findings,wu2016google,crego2016systran,junczys2016neural}.
The progress was largely driven by the encoder-decoder framework \citep{sutskever2014sequence,cho2014learning} and typically supplemented with an attention mechanism \citep{bahdanau2014neural,luong2015effective}.

Compared to the traditional phrase-based systems \citep{koehn2009statistical}, neural machine translation (NMT) requires large amounts of data in order to reach high performance \citep{koehn2017six}.
Using NMT in a multilingual setting exacerbates the problem by the fact that given $k$ languages translating between all pairs would require $O(k^2)$ parallel training corpora (and $O(k^2)$ models).

In an effort to address the problem, different multilingual NMT approaches have been proposed recently.
\citet{luong2015multi, firat2016multi} proposed to use $O(k)$ encoders/decoders that are then intermixed to translate between language pairs.
\citet{johnson2016google} proposed to use a single model and prepend special symbols to the source text to indicate the target language, which has later been extended to other text preprocessing approaches \citep{ha2017effective} as well as language-conditional parameter generation for encoders and decoders of a single model \citep{platanios2018contextual}.

\input{figures/agreement-illustration}

\citet{johnson2016google} also show that a single multilingual system could potentially enable \textit{zero-shot} translation, \ie, it can translate between language pairs not seen in training.
For example, given 3 languages---German (\De), English (\En), and French (\Fr)---and training parallel data only for (\De, \En) and (\En, \Fr), at test time, the system could additionally translate between (\En, \Fr).


Zero-shot translation is an important problem.
Solving the problem could significantly improve data efficiency---a single multilingual model would be able to generalize and translate between any language pair per request after being trained only on $O(k)$ parallel corpora.
However, performance on zero-shot tasks is often unstable and significantly lags behind the supervised directions.
Moreover, attempts to improve zero-shot performance by fine-tuning~\cite{firat2016zero,sestorain2018zero} may negatively impact other directions.

In this work, we take a different approach and aim to improve the training procedure of \citet{johnson2016google}.
First, we analyze multilingual translation problem from a probabilistic perspective and define the notion of \textit{zero-shot consistency} that gives insights as to why the vanilla training method may not yield models with good zero-shot performance.
Next, we propose a novel training objective and a modified learning algorithm that aim to improve zero-shot translation by achieving consistency via agreement-based learning \citep{liang2006alignment,liang2008agreement}.
Our training procedure encourages the  model to  produce  equivalent  translations  of  parallel training sentences into an auxiliary, third language (Figure~\ref{fig:agreement-illustration}) and is provably zero-shot consistent.
In addition, we make a simple change to the standard neural decoder to make the agreement losses end-to-end  differentiable.

We conduct experiments on the IWSLT 2017 \citep{mauro2017overview}, UN corpus \citep{ziemski2016united}, and Europarl \citep{koehn2017europarl} showing  that  agreement-based learning results in up to +3 BLEU zero-shot improvement over the baseline, compares favorably (up to +2.4 BLEU) to other approaches in the literature \citep{cheng2017joint, sestorain2018zero}, is competitive with pivoting, and does not lose in performance on supervised directions.





==> sections/scratch.tex <==
\subsection{Consistent multilingual models}
\label{sec:consistent-multilingual-nmt}

As we noted, directly optimizing \eqref{eq:basic-multilingual-nmt-objective} is generally unlikely to get us a consistent NMT system.
On the other hand, we can apply certain post-processing to get zero-shot consistent translations.

\textbf{Pivoting.}
As long as we can get from any source to any target language along the supervised directions in the translation graph, we can ``pivot'' on an intermediate language and construct a pipeline model for any zero-shot direction.
For example, we can translate from $\Es$ to $\Fr$ through $\En$ (Figure~\ref{fig:translation-graph}):
\begin{equation}
    \label{eq:pivot-estimator}
    \begin{split}
        \MoveEqLeft \probh{\xv_\Fr \mid \xv_\Es} = \\
        & \sum_{\xv_\En} \prob[\hat \theta]{\xv_\Fr \mid \xv_\En} \prob[\hat \theta]{\xv_\En \mid \xv_\Es}
    \end{split}
\end{equation}
The sum over the pivot translations, $\xv_\En$, is usually substituted with the best translation, $\hat \xv_\En \approx \argmax_{\xv_\En} \prob[\hat \theta]{\xv_\En \mid \xv_\Es}$.
We can claim that pivoting is provably zero-shot consistent with respect to the cross-entropy loss under certain assumptions:
\begin{proposition}[Consistency of pivoting]
If the $\En \rightarrow \Fr$ loss is bounded as:
\begin{equation}
\ep[\xv_\En, \xv_\Fr]{\log \prob[\theta]{\xv_\Fr \mid \xv_\En}} \leq \varepsilon
\end{equation}
and the following bound holds for the $\Es \rightarrow \En$ model:
\begin{equation*}
\frac{\prob[\theta]{\xv_\En \mid \xv_\Es}}{\prob{\xv_\En \mid \xv_\Es, \xv_\Fr}} \leq \delta,\, \xv_\En, \xv_\Es \sim \prob{\xv_\En, \xv_\Es}
\end{equation*}
Then the expected loss of the pivoting model is 
\end{proposition}

\textbf{Distillation.}
Another approach to ensure consistency is distillation~\citep{kim2016sequence,chen2017teacher}.
The setup is similar to pivoting, but instead of using a chain-like translator (\eg, $L_2 \rightarrow L_1 \rightarrow L_3$), we can fine-tune zero-shot models by imitating the supervised models.
For instance, given $(\xv_1, \xv_2) \in \Cc_{12}$, we can fine-tune $\prob[\theta]{\xv_3 \mid \xv_2}$ by trying to match $\prob[\theta]{\xv_3 \mid \xv_1}$.
There are a few downsides to the approach: (i) it is multi-stage (\ie, first train, then fine-tune), (ii) requires fine-tuning each zero-shot direction separately, (iii) fine-tuning, if done on top of a model with shared encoders and decoders, it might weaken supervised directions.


